Learning Representations and Agents for Information Retrieval

A goal shared by artificial intelligence and information retrieval is to create an oracle, that is, a machine that can answer our questions, no matter how difficult they are. A more limited, but still instrumental, version of this oracle is a question-answering system, in which an open-ended question is given to the machine, and an answer is produced based on the knowledge it has access to. Such systems already exist and are increasingly capable of answering complicated questions. This progress can be partially attributed to the recent success of machine learning and to the efficient methods for storing and retrieving information, most notably through web search engines. One can imagine that this general-purpose question-answering system can be built as a billion-parameters neural network trained end-to-end with a large number of pairs of questions and answers. We argue, however, that although this approach has been very successful for tasks such as machine translation, storing the world's knowledge as parameters of a learning machine can be very hard. A more efficient way is to train an artificial agent on how to use an external retrieval system to collect relevant information. This agent can leverage the effort that has been put into designing and running efficient storage and retrieval systems by learning how to best utilize them to accomplish a task. ...

==> future.tex <==
\chapter{A Future Direction}
\label{chap:future}

\todo{Write a introduction.}

\section{Suggesting the Bibliography of a Future High-Impact Paper with Minimal Information}

\begin{figure}
%\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=0.8\columnwidth]{imgs/citations_histogram}}
\vskip -0.1in
\caption{The histogram of citations of the Open Research Corpus. The main motivation for the proposed task comes from the observation that highly-cited papers are scarce, as less than 2.5\% of the papers have more than 50 citations.}
\label{fig:citations_histogram}
\end{center}
%\vskip -4mm
\end{figure}

The goal of creating an automated scientist has been the dream of many~\cite{waltz2009automating, lloyd2014automatic, schmidhuber2003godel}. This machine would be able to invent a theory to explain an observation, design experiments to validate it, and repeat this cycle until one of the versions of the theory agrees with the experiments and observations.

Throughout this thesis, we presented methods for improving systems that help users find answers to their questions. The goal of the machine is achieved if the provided answer is correct. To develop an automated scientist, however, the important functionality of proposing novel and relevant ideas is still missing.

Here, we propose a new task towards this objective. The goal is to gather scientific works that together can serve as a basis to create a high-impact work. Our motivation for proposing this task comes from the fact that papers with a high number of citations are scarce. For example, among the 20 million scientific papers from computer science, neuroscience, and biomedicine in the Open Resource Corpus~\cite{ammar2018construction}, less than 2.5\% have more than 50 citations (Figure~\ref{fig:citations_histogram}). We hope to improve this statistic through the proposed task and the systems developed for it.

Since the impact of a newly created work may not be easily verifiable in a near future, we make simplifications to carry out this task in a concrete way. We start by defining the impact of scientific work as the number of times other works cite it.

Different from most bibliography suggestion methods, which target on finding works related to an ongoing work~\cite{woodruff2000enhancing, gori2006research, mcnee2002recommending, agarwal2005research}, we design the task so that the suggestion mechanism has access to minimal information about the work in progress. More precisely, the machine receives as input a scientific work that the author plans to include in the bibliography of a future work. This incentivizes the machine to freely explore the desired topic and possible ideas of interest without sticking to similar works only.

In summary, we propose a task whose goal is to suggest a bibliography that will increase the likelihood of a paper having a high-impact while requiring minimal effort from the author's perspective into providing input information.

%Another way to view this task is that of predicting the evolution of the graph of citations, but focusing only on the papers that will have a high number of citations.

\subsection{Related Work}

The proposed task is mainly related to two research topics: bibliography suggestion and scientific impact prediction. 

Automated bibliography suggestion has been a topic of intense study~\cite{woodruff2000enhancing, gori2006research, mcnee2002recommending, agarwal2005research}. Most of the existing methods use the partial~\cite{gori2006research} or full text~\cite{mcnee2002recommending} of an ongoing work as an input.\footnote{A notable exception is the \href{www.semanticscholar.org}{Semantic Scholar search engine}, which accepts short queries to perform the search} This implies that the author must have some of the ongoing work already described before starting looking for related literature. Our method alleviates this requirement by using as an input an existing paper that expresses the topic of interest of the author.
Moreover, existing methods focus on maximizing retrieval of related literature of a given paper, whereas our task aims at maximizing retrieval of the literature of a yet to exist high-impact work.

In the area of impact prediction, the closest works to ours are those from~\citet{dong2015will} and~\citet{dong2016can}, in which paper content and information about the authors are used to predict the impact of a paper in the authors' h-index. Other works focus on predicting the impact of new scientific terms~\cite{mckeown2016predicting} or the future impact of scientists based on their publications, co-authors, and affiliations~\cite{acuna2012future}. Our goal is different as we focus on suggesting the literature that will serve as a base for the creation of a high-impact work. Therefore, the content of the new work and the scientific performance of the authors are dispensable.

\subsection{A New Dataset: high-impact BIbliography SuggestiON (BISON)}

We construct the dataset for the proposed task using the Open Resource Corpus as the source for high-impact papers and their bibliographies. First, we select all papers that have more than 50 citations as the high-impact papers (yellow paper in Figure~\ref{fig:bib_pred_task}). For each, we randomly select one of the papers in its bibliography (green paper) and use the concatenation of its title and abstract as the input paper. The remaining bibliography is used as ground-truth target documents (blue papers). Our final corpus consists of titles and abstracts of all papers except the high-impact ones since these are only used to obtain pairs of input and ground-truth papers.

We end up with approximately 116,000 pairs of input and target papers that we split into 96K, 10K and 10K examples for training, development and test sets, respectively. Statistics of the dataset are shown in Table~\ref{tab:bib_pred_statistics}.

\begin{figure}
%\vskip 0.2in
\begin{center}
\includegraphics[width=0.7\columnwidth]{imgs/bibliography_prediction_task}
\vskip -0.1in
\caption{Illustration of the proposed task using computer vision papers as examples. The arrows correspond to citations. The goal is to predict the bibliography of a future highly-cited work without having access to any information about its content. The green paper (SIFT~\cite{lowe2004distinctive}) is the paper of interest, and it is given as an input. The output should be the blue papers (ImageNet~\cite{deng2009imagenet} and ConvNet~\cite{lecun1989backpropagation}) as these \textit{will be} cited by a future high-impact paper (yellow paper, AlexNet~\cite{krizhevsky2012imagenet}). The high-impact paper is not included in the corpus available to the prediction system; only its bibliography is used to define input and ground-truth target papers.}
\label{fig:bib_pred_task}
\end{center}
%\vskip -4mm
\end{figure}



\begin{table}
%\vskip 0.05in
\begin{center}
\begin{footnotesize}
\begin{tabular}{l|c}
 & BISON \\
\noalign{\vskip 1mm}
\hline
\noalign{\vskip 1mm}
Total Number of Papers in the Corpus & 20.3M\\
Avg. Paper Length (\# chars, Title+Abstract only$^{\star}$) & 1,180 \\
Avg. Input Paper Length (\# chars, Title+Abstract) & 1,250 \\
Avg. Input Paper Length (\# chars, Title only) & 89 \\
Avg. Number of Target Papers per Input Paper & 26 \\
\end{tabular}
\end{footnotesize}
\end{center}
\vskip -1mm
\caption{Statistics of the proposed BISON dataset. $^{\star}$We do not use the full documents mostly due to missing or broken download links.}
\label{tab:bib_pred_statistics}
%\vskip 4mm
%\vspace{-4mm}
\end{table}

\subsection{Preliminary Experiments}

Here, we briefly describe preliminary experiments. For this retrieval task, we use the baseline system (Lucene) and the reformulation methods (RL-RNN and RL-10-Sub) described in Chapters~\ref{chap:query_reformulation} and~\ref{chap:scaling_up_query_reformulation}. We use as an input query only the title of the input paper. 

Table~\ref{tab:results_bison} shows the results. The reformulation methods perform better than the baseline search engine. Nevertheless, the numbers across all metrics indicate that there is room for improvement in the proposed task.

\begin{table}
%\vskip 0.05in
\begin{center}
\begin{footnotesize}
\begin{tabular}{l|ccccc}
 & Recall@40 & MAP & R-Precision & MRR & NDCG\\
\noalign{\vskip 1mm}
\hline
\noalign{\vskip 1mm}
Lucene & 5.1 & 1.29 & 2.83 & 10.1 & 4.2 \\
\noalign{\vskip 1mm}
\hline
\noalign{\vskip 1mm}
RL-RNN & 6.2 & 1.54 & 3.25 & 11.4 & 4.9\\
RL-10-Sub (Pretrained) & 7.3 & 1.80 & 3.84 & 13.0 & 5.7\\
\end{tabular}
\end{footnotesize}
\end{center}
\vskip -1mm
\caption{Preliminary results on the test set of the BISON dataset.}
\label{tab:results_bison}
%\vskip 4mm
%\vspace{-4mm}
\end{table}


\pagebreak
